A Pixel-Level Meta-Learner for Weakly Supervised Few-Shot Semantic Segmentation

Few-shot semantic segmentation addresses the learning task in which only few images with ground truth pixel-level labels are available for the novel classes of interest. One is typically required to collect a large mount of data (i.e., base classes) with such ground truth information, followed by meta-learning strategies to address the above learning task. When only image-level semantic labels can be observed during both training and testing, it is considered as an even more challenging task of weakly supervised few-shot semantic segmentation. To address this problem, we propose a novel meta-learning framework, which predicts pseudo pixel-level segmentation masks from a limited amount of data and their semantic labels. More importantly, our learning scheme further exploits the produced pixel-level information for query image inputs with segmentation guarantees. Thus, our proposed learning model can be viewed as a pixel-level meta-learner. Through extensive experiments on benchmark datasets, we show that our model achieves satisfactory performances under fully supervised settings, yet performs favorably against state-of-the-art methods under weakly supervised settings.

==> tabs/pascal_15shot_fw.tex <==
% \begin{table}[!tp]
%     \centering
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{cccccccccccccccc} 
%         \hline\hline
%         \multicolumn{2}{c}{\multirow{2}{*}{Method}} & \multicolumn{6}{c}{1-shot}                                               & \multicolumn{6}{c}{5-shot}                                        \\ 
%         \cmidrule(lr){3-8}\cmidrule(lr){9-14}
%         \multicolumn{2}{c}{}                        & $5^0$  & $5^1$  & $5^2$  & $5^3$  & Mean & \multicolumn{1}{c}{$\Delta$ } & $5^0$  & $5^1$  & $5^2$  & $5^3$  & Mean & $\Delta$               \\ 
%         \Xhline{2\arrayrulewidth}
%         \multirow{2}{*}{PANet~\cite{panet}} & \textit{f}         & ---   & ---   & ---   & ---   & 45.1 & \multirow{2}{*}{18.9}         & ---   & ---   & ---   & ---   & 53.1 & \multirow{2}{*}{16.5}  \\ 
%         \cline{2-2}
%                               & \textit{w}         & 24.5   & 33.6   & 26.3   & 20.3   & 26.2 &                               & 35.3   & 44.9   & 37.8   & 28.2   & 36.6 &                        \\ 
%         \hline
%         \multirow{2}{*}{Ours}  & \textit{f}         & 36.5   & 51.8   & 48.5   & 38.9   & 43.9 & \multirow{2}{*}{\textbf{6.2}}          & 41.4   & 57.9   & 55.1   & 42.9   & 49.3 & \multirow{2}{*}{\textbf{6.3}}   \\ 
%         \cline{2-2}
%                               & \textit{w}         & 31.5   & 46.7   & 41.4   & 31.2   & \textbf{37.7} &                               & 37.4   & 52.6   & 45.6   & 36.6   & \textbf{43.0} &                        \\
%         \hline\hline
%         \end{tabular}
%     }
%     \caption{Quantitative results of 2-way segmentation on the PASCAL-$5^i$ dataset.}
%     \label{tab:pascal2}
% \end{table}

==> tabs/pascal_all.tex <==
% \begin{table*}[!tp]
%     \centering
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{ccccccccccccc} 
%         \hline\hline
%         \multirow{2}{*}{Method} & \multicolumn{6}{c}{\textbf{1-shot}} & \multicolumn{6}{c}{\textbf{5-shot}} \\ 
%         \cmidrule(lr){2-7}\cmidrule(lr){8-13}
%         {} & Split-0  & Split-1  & Split-2  & Split-3  & Mean & $\Delta$ & Split-0  & Split-1  & Split-2  & Split-3 & Mean & $\Delta$ \\ 
%         \Xhline{2\arrayrulewidth}
%         % \multicolumn{9}{c}{\textbf{1-way}} \\
%         \textbf{1-way} \\
%         Co-att~\cite{coattention} & 49.5 & 65.5 & 50.0 & 49.2 & 53.5 & --- & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & 51.7 & --- \\
%         % \hline
%         AMP~\cite{amp} & 41.9 / 10.6 & 50.2 / 14.1 & 46.7 / 7.6 & 34.7 / 10.9 & 43.4 / 10.8 & 32.6 \\
%         % \hline
%         PANet~\cite{panet} & {42.3} / {25.7} & {58.0} / {33.4} & {51.1} / {28.8} & {41.2} / {20.7} & {48.1} / {27.1} & 21.0 & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & {55.7} / {37.7} & 18.0 \\
%         % \hline
%         Ours & {38.3} / {36.5} & {57.6} / {51.7} & {54.0} / {45.9} & {40.1} / {35.6} & {47.5} / {\textbf{42.4}} & \textbf{5.1} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & {50.6} / {\textbf{45.5}} & \textbf{5.1} \\
%         \hline
%         \textbf{2-way} \\
%         PANet~\cite{panet} & \phantom{0.}--- / {24.5} & \phantom{0.}--- / {33.6} & \phantom{0.}--- / {26.3} & \phantom{0.}--- / {20.3} & {45.1} / {26.2} & 18.9 & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & {53.1} / {36.6} & 16.5 \\
%         % \hline
%         Ours & {36.5} / {31.5} & {51.8} / {46.7} & {48.5} / {41.4} & {38.9} / {31.2} & {43.9} / {\textbf{37.7}} & \textbf{6.2} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & \phantom{0.}--- / ---\phantom{0.} & {49.3} / {\textbf{43.0}} & \textbf{6.3} \\
%         \hline\hline
%     \end{tabular}
%     }
%     \caption{Quantitative evaluation on PASCAL-$5^i$ in terms of mean-IoU. {Red} and {Blue} indicate results under fully supervised and extremely weakly supervised settings, respectively. $\Delta$ denotes the performance drop from supervised to weakly supervised settings. Note that \cite{coattention} is trained in a different setting and should be considered as a performance upper bound.
%     %which confirms that our model is preferable for few-shot semantic segmentation if only class label is observed.
%     }
%     \label{tab:pascal}
% \end{table*}

==> tabs/pascal_coco.tex <==
% \begin{table*}[]
%   \centering

%   \begin{subtable}[b]{.5\linewidth}
%     \centering
%       \resizebox{.97\linewidth}{!}{%
%       \begin{tabular}{ccccccccc} 
%         \hline\hline
%         \multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{1-shot}}                                               & \multicolumn{2}{c}{\textbf{5-shot}}                                        \\ 
%         \cmidrule(lr){2-3}\cmidrule(lr){4-5}
%         {} & Mean & $\Delta$ & Mean & $\Delta$               \\ 
%         \Xhline{2\arrayrulewidth}
%         % \multicolumn{9}{c}{\textbf{1-way}} \\
%         \textbf{1-way} \\
%         Co-att~\cite{coattention} & 53.5 & --- & 51.7 & --- \\
%         % \hline
%         AMP~\cite{amp} & 43.4 / 10.8 & 32.6 & 46.9 / 14.7 & 32.2 \\
%         % \hline
%         PANet~\cite{panet} & 48.1 / 27.1 & 21.0 & 55.7 / 37.7 & 18.0 \\
%         % \hline
%         Ours & 47.5 / \textbf{42.4} & \textbf{5.1} & 50.6 / \textbf{45.6} & \textbf{5.0} \\
%         \hline
%         \textbf{2-way} \\
%         PANet~\cite{panet} & 45.1 / 26.2 & 18.9 & 53.1 / 36.6 & 16.5 \\
%         % \hline
%         Ours & 43.9 / \textbf{37.7} & \textbf{6.2} & 49.3 / \textbf{43.0} & \textbf{6.3} \\
%         \hline\hline
%       \end{tabular}
%       }
%     \caption{PASCAL-$5^i$}
%     \label{tab:pascal}
%   \end{subtable}%
%   %
%   \begin{subtable}[b]{.5\linewidth}
%     \centering
%       \resizebox{.97\linewidth}{!}{%
%       \begin{tabular}{ccccccccc} 
%         \hline\hline
%         \multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{1-shot}}                                               & \multicolumn{2}{c}{\textbf{5-shot}}                                        \\ 
%         \cmidrule(lr){2-3}\cmidrule(lr){4-5}
%         {} & Mean & $\Delta$ & Mean & $\Delta$               \\ 
%         \Xhline{2\arrayrulewidth}
%         % \multicolumn{9}{c}{\textbf{1-way}} \\
%         \textbf{1-way} \\
%         PANet~\cite{panet} & 20.9 / 8.0 & 12.9 & 29.7 / 13.9 & 15.8 \\
%         % \hline
%         Ours & 19.7 / \textbf{17.0} & \textbf{2.7} & 27.0 / \textbf{17.5} & \textbf{9.5} \\
%         \hline
%         \textbf{2-way} \\
%         Ours & 11.5 / \textbf{11.1} & \textbf{0.4} & 14.8 / \textbf{11.9} & \textbf{2.9} \\
%         \hline\hline
%       \end{tabular}
%       }
%     \caption{MS COCO 2014}
%     \label{tab:coco}
%   \end{subtable}%

%   \caption{Performance evaluation on (a) PASCAL-$5^i$ and (b) MS COCO in terms of mean-IoU. The numbers before and after `/' indicate results under fully and extremely weakly supervised settings, respectively. $\Delta$ denotes the performance drop between the two settings. Note that \cite{coattention} considers a weakly supervised setting but still observes ground truth pixel-level masks during training.}
%   \label{tab:pascal_coco}
% \end{table*}

==> tabs/sampling.tex <==
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \includestandalone[width=\linewidth]{figs/sample}
  \captionof{figure}{Performances of support pixel sampling with varying $n_s$ on PASCAL-$5^i$. Note that $n_s$ denotes the number of support pixels sampled from each category for semantic segmentation.}
  \label{fig:sample}
\end{minipage}
